Electric currents in infinite networks

In this survey, we present the basic facts about conduction in infinite networks. This survey is based on the work of Flanders, Zemanian, and Thomassen, who developed the theory of infinite networks from scratch. Here we show how to get a more complete theory by paralleling the well-developed theory of conduction on open Riemann surfaces. Like Flanders and Thomassen, we take as a test case for the theory the problem of determining the resistance across an edge of a d-dimensional grid of 1-ohm resistors.

==> net_dot_bib <==
@book{ahlforsSario:riemannSurfaces,
	author =	"L. V. Ahlfors and L. Sario",
	address =	"Princeton, N. J.",
	year =		"1960",
	publisher =	"Princeton Univ. Press",
	title =		"{R}iemann Surfaces"
}

@article{avez:ohp,
	author =	"A. Avez",
	title =		"Th\'{e}or\`{e}me de {C}hoquet-{D}eny pour les groupes de croissance non exponentielle",
	journal =	"C. R. Acad. Sciences Paris S\'{e}r. A",
	volume =	"279",
	year =		"1974",
	pages =		"25-28"
}

@book{bollobas:graph,
	author =	"B. Bollob\'{a}s",
	title =		"Graph Theory",
	publisher =	"Springer",
	address =	"New York",
	year =		"1979"
}

@book{doyleSnell:carus,
	author =	"P. G. Doyle and J. L. Snell",
	address =	"Washington, D. C.",
	title =		"Random Walks and Electric Networks",
	publisher =	"Mathematical Association of America",
	year =		"1984"
}

@article{flanders:infinite,
	author =	"H. Flanders",
	title =		"Infinite Networks: {I}---resistive networks",
	journal =	"IEEE Trans. Circuit Theory",
	volume =	"18",
	year =		"1971",
	pages =		"326-331"
}

@article{flanders:infiniteGrid,
	author =	"H. Flanders",
	title =		"Infinite Networks: {II}---resistances in an infinite grid",
	journal =	"J. Math. Anal. Appl.",
	volume =	"40",
	year =		"1972",
	pages =		"30-35"
}

@incollection{foster:average,
	author =	"R. M. Foster",
	title =		"The average impedance of an electrical network",
	pages =		"333-340",
	booktitle =	"Contributions to Applied Mechanics (Reissner Anniversary Volume)",
	publisher =	"Edwards Bros.",
	address =	"Ann Arbor, Mich.",
	year =		"1949"
}

@article{foster:extension,
	author =	"R. M. Foster",
	title =		"An extension of a network theorem",
	journal =	"IRE Trans. Circuit Theory",
	volume =	"8",
	year =		"1961",
	pages =		"75-76"
}

@article{gromov:polynomial,
	author =	"M. Gromov",
	title =		"Groups of polynomial growth and expanding maps",
	journal =	"Inst. Hautes \'{E}tudes Sci. Publ. Math.",
	volume =	"53",
	year =		"1981",
	pages =		"53-78"
}

@article{kirchhoff:gleichungen,
	author =	"G. Kirchhoff",
	title =		"{U}eber die {A}ufl{\"{o}}sung der {G}leichungen,
				auf welche man bei der {U}ntersuchung
				der linearen {V}ertheilung {G}alvanischer
				{S}tr{\"{o}}me gef{\"{u}}hrt wird",
	journal =	"Ann. Phys. Chem.",
	volume =	"72",
	year =		"1847",
	pages =		"497-508"
}

@book{maxwell:treatise,
	author =	"J. C. Maxwell",
	title =		"Treatise on Electricity and Magnetism",
	edition =	"Third",
	publisher =	"Clarendon",
	address =	"Oxford",
	year =		"1891"
}

@book{rodinSario:principal,
	author =	"B. Rodin and L. Sario",
	title =		"Principal Functions",
	publisher =	"D. van Nostrand",
	address =	"Princeton, N. J.",
	year =		"1968"
}

@book{spitzer:principles,
	author =	"F. Spitzer",
	title =		"Principles of Random Walk",
	edition =	"Second",
	publisher =	"Springer",
	address =	"New York",
	year =		"1976"
}

@unpublished{thomassen:infinite,
	author =	"C. Thomassen",
	title =		"Resistances and currents in infinite electrical networks",
	note =		"preprint"
}

@article{varopoulos:polya,
	author =	"N. Th. Varopoulos",
	title =		"Th\'{e}orie du potentiel sur des groupes et des vari\'{e}t\'{e}s",
	journal =	"C. R. Acad. Sciences Paris S\'{e}r. I",
	volume =	"302",
	year =		"1986",
	pages =		"203-205"
}

@book{weinberg:network,
	author =	"L. Weinberg",
	title =		"Network Analysis and Synthesis",
	publisher =	"McGraw-Hill",
	address =	"New York",
	year =		"1962"
}

@article{zemanian:infinite,
	title =		"Infinite electrical networks",
	journal =	"Proc. IEEE",
	author =	"A. H. Zemanian",
	volume =	"64",
	year =		"1976",
	pages =		"6-17"
}

